Reinforcement Learning Your Way: Agent Characterization through Policy Regularization

The increased complexity of state-of-the-art reinforcement learning (RL) algorithms have resulted in an opacity that inhibits explainability and understanding. This has led to the development of several post-hoc explainability methods that aim to extract information from learned policies thus aiding explainability. These methods rely on empirical observations of the policy and thus aim to generalize a characterization of agents' behaviour. In this study, we have instead developed a method to imbue a characteristic behaviour into agents' policies through regularization of their objective functions. Our method guides the agents' behaviour during learning which results in an intrinsic characterization; it connects the learning process with model explanation. We provide a formal argument and empirical evidence for the viability of our method. In future work, we intend to employ it to develop agents that optimize individual financial customers' investment portfolios based on their spending personalities.

==> source/statements.tex <==

\vspace{6pt}

\authorcontributions{Conceptualization, C.M. and C.O.; methodology, C.M.; software, C.M.; validation, C.M.; formal analysis, C.M.; investigation, C.M.; resources, C.M.; data curation, C.M.; writing---original draft preparation, C.M.; writing---review and editing, C.O. and C.M; visualization, C.M.; supervision, C.O.; project administration, C.M.; funding acquisition, C.M. and C.O.; All authors have read and agreed to the published version of the manuscript.}

\funding{This research was partially funded by The Norwegian Research Foundation, project number 311465.}

% \acknowledgments{}

\conflictsofinterest{The authors declare no conflict of interest. The funders had no role in the design of the study, in the collection, analyses, or interpretation of data, in the writing of the manuscript, or in the decision to publish the results.} 
